Real-Time Parallel Trajectory Optimization with Spatiotemporal Safety Constraints for Autonomous Driving in Congested Traffic

Multi-modal behaviors exhibited by surrounding vehicles (SVs) can typically lead to traffic congestion and reduce the travel efficiency of autonomous vehicles (AVs) in dense traffic. This paper proposes a real-time parallel trajectory optimization method for the AV to achieve high travel efficiency in dynamic and congested environments. A spatiotemporal safety module is developed to facilitate the safe interaction between the AV and SVs in the presence of trajectory prediction errors resulting from the multi-modal behaviors of the SVs. By leveraging multiple shooting and constraint transcription, we transform the trajectory optimization problem into a nonlinear programming problem, which allows for the use of optimization solvers and parallel computing techniques to generate multiple feasible trajectories in parallel. Subsequently, these spatiotemporal trajectories are fed into a multi-objective evaluation module considering both safety and efficiency objectives, such that the optimal feasible trajectory corresponding to the optimal target lane can be selected. The proposed framework is validated through simulations in a dense and congested driving scenario with multiple uncertain SVs. The results demonstrate that our method enables the AV to safely navigate through a dense and congested traffic scenario while achieving high travel efficiency and task accuracy in real time.

==> Sections/related_work.tex <==
\section{Related works} 
\label{sec:related_works}
 Extensive research efforts have focused on facilitating the safe and efficient interaction between the EV and other SVs ~\cite{planning_and_dm_for_avs_2018,paden2016survey}. To enable efficient replanning in traffic flow, A sampling-based motion planner is proposed to generate a smooth, jerk-optimal polynomial trajectory for the EV in~\cite{werling2012optimal}. This work aims to generate multiple candidate quartic trajectories towards different goals and rank them based on a cost function that considers various constraints. However, this planner cannot optimize the sampled trajectory to satisfy state and control input constraints, which is hard to generate a safe and feasible trajectory in congested traffic. To address this issue, the piecewise polynomials represented by Bézier curves~\cite{moon2014trajectory} and clothoid curves~\cite{vorobieva2014automatic} are smooth and easily optimized to meet state and control constraints. Hence, intensive works exist in optimized-based planning based on polynomial curves~\cite{xu2021autonomous,wang2021game,han2022differential}. A computational-efficient recurrent spline trajectory optimization method is proposed to generate an obstacle-free path in the static environment for autonomous driving~\cite{xu2021autonomous}, whereas it does not consider dynamic SVs in its framework. Considering dynamic obstacles, these planners leverage the differential flatness property of the bicycle kinematic model to generate smooth and feasible trajectories for the EV to safely interact with other SVs in real-time~\cite{wang2021game,han2022differential}. While these polynomial-based the planner can generate safe and smooth trajectories, they cannot fully exploit 
exploit the actuator potential of AVs with nonholonomic constraints and higher nonlinearity, leading to sub-optimal control policies~\cite{romero2022model}. 

On the other hand, the optimal control frameworks, such as constrained differential dynamic programming (DDP)\cite{chen2019autonomous} and model predictive control (MPC)\cite{mayne2014model}, can naturally incorporate system models and have been widely used in autonomous driving applications. 
Constrained iterative linear quadratic regulators (iLQR), a DDP method, have been developed to handle nonlinear constraints of system dynamics and non-convexity of obstacle avoidance constraints for AVs in \cite{ chen2019autonomous,chen2017constrained,pan2020safe}.
However, these optimizations require an obstacle-free reference trajectory at the first iteration, which is generated using iLQR with a logarithmic barrier function. Alternatively, MPC approaches can consider system constraints and anticipate the future state in its optimization framework, which has been widely utilized in autonomous driving~\cite{ ji2016path, wurts2018collision, zeng2021safety, yin2022trajectory}. The safety term is encoded as a distant term to obstacles into the objective function of MPC to avoid a potential collision with SVs to realize aggressive lane change maneuvers in~\cite{ wurts2018collision}. 
To realize proactive collision avoidance, the control barrier function~\cite{ames2019control} has been utilized in~\cite{zeng2021safety} to enforce the safety of the EV when overtaking its front vehicle.  
However, the computationally burdensome optimization process, particularly the inverse of the Hessian matrix~\cite{ma2022local}, remains a limiting factor for real-time replanning within autonomous driving planning horizons of 5 to 10 seconds\cite{sadat2019jointly}.
To address these issues, researchers have turned to the alternating direction method of multipliers (ADMM)~\cite{boyd2011distributed} to reduce the computational burden of optimization processes caused by the nonlinearity and non-convexity of the trajectory optimization problem~\cite{ma2022alternating, han2023rda}.  
The ADMM splits the optimization problem into several sub-problems that can be efficiently solved within the iLQR~\cite{ma2022alternating} or MPC framework~\cite{han2023rda}. However, existing works assign a predefined constant motion model to the SVs~\cite{ma2022alternating} or neglect dynamic obstacles~\cite{han2023rda}, which can lead to safety concerns in dynamic, congested traffic flow due to model mismatches and uncertain multi-mode behaviors of SVs. Considering uncertain behaviors, the branch MPC approaches have been developed for safe and efficient interaction with uncertain SVs for the EV in ~\cite{adajania2022multi, chen2022interactive}. The batch MPC~\cite{adajania2022multi} utilizes alternating minimum to parallelly optimized multiple trajectories and evaluates them to obtain the optimal trajectory in a traffic flow where  SVs exhibit multi-modal behaviors, whereas it doesn't account for the driving consistency when evaluating the candidate trajectories, which may result in frequent lane change in dense and dynamic congested Traffic.
  

==> Sections/results.tex <==
 
